Analyzing and Debugging Normative Requirements via Satisfiability Checking

As software systems increasingly interact with humans in application domains such as transportation and healthcare, they raise concerns related to the social, legal, ethical, empathetic, and cultural (SLEEC) norms and values of their stakeholders. Normative non-functional requirements (N-NFRs) are used to capture these concerns by setting SLEEC-relevant boundaries for system behavior. Since N-NFRs need to be specified by multiple stakeholders with widely different, non-technical expertise (ethicists, lawyers, regulators, end users, etc.), N-NFR elicitation is very challenging. To address this challenge, we introduce N-Check, a novel tool-supported formal approach to N-NFR analysis and debugging. N-Check employs satisfiability checking to identify a broad spectrum of N-NFR well-formedness issues (WFI), such as conflicts, redundancy, restrictiveness, insufficiency, yielding diagnostics which pinpoint their causes in a user-friendly way that enables non-technical stakeholders to understand and fix them. We show the effectiveness and usability of our approach through nine case studies in which teams of ethicists, lawyers, philosophers, psychologists, safety analysts, and engineers used N-Check to analyse and debug 233 N-NFRs comprising 62 issues for the software underpinning the operation of systems ranging from assistive-care robots and tree-disease detection drones to manufacturing collaborative robots.

==> Archive/introduction-jun-28.tex <==
\section{Introduction}
\label{sec:introduction}
% Context: normative requirements
Software systems interacting with humans become prevalent in domains such as transportation~\cite{Pham-et-al-16,Nagatani-et-al-21}, health and social care~\cite{Salceda-05,Laursen-et-al-22}. 
% example
For example, in the domain of healthcare~\cite{Salceda-05,Laursen-et-al-22}, helper robots are being used to assist patients with dressing. 
The deployment of such systems raises significant concerns in the realms of social, legal, ethical, empathetic, and cultural aspects (referred to as SLEEC) that must be addressed during development~\cite{townsend-et-al-2022, Bremner2019DFW, Burton2020HMP}. 
% example
% For instance, to avoid that a dressing robot reveals a patient's personal information. 
For instance, a helper robot might accidentally reveal patients' personal information without patients' consent.
To tackle these concerns effectively, normative requirements (\nNFRs) are defined, which are non-functional system requirements (NFRs) based on social, ethical, legal, cultural, or other relevant factors, \red{which restrict the acceptable range of system behavior that excludes the concerns}. 
% example
For instance, \nNFRs{} for a helper robot may specify that the patient's well-being and privacy are prioritized by promptly completing the dressing task, especially when the patient is underdressed. 
\red{\nNFRs{} are then used to inform all subsequent software engineering (SE) activities, such as design and architecture, testing and validation, and compliance and regulation. 
It is therefore important to carefully elicit them, and to validate them at an early stage, to avoid propagation of mistakes.}

\red{Similarly to non-functional requirements, three main types of inconsistencies — conflict, restrictiveness, and sufficiency — can arise during the elaboration of normative requirements. 
Additionally, a potential source of inconsistency, namely redundancy, can also occur. 
In the following, we will describe each of these issues.}

% Conflicting rules
\boldparagraph{Conflicting \nNFRs}
Typically, \nNFRs{} can be specified by multiple stakeholders independently~\cite{Lamsweerde-Darimont-Letier-98}. 
These stakeholders have different concerns, priorities, and responsibilities. 
Consequently, a common problem in non-functional requirements elicitation is the occurrence of \emph{conflicting} requirements~\cite{Shah-et-al-21}. 
In the context of \nNFRs{}, where multiple factors must be considered simultaneously (e.g., social and legal factors), conflicting requirements can also arise from different norms and factors~\cite{townsend-et-al-2022}, even if the requirements are elicited by a single stakeholder, such as a SLEEC expert.
% example
For the helper robot, the \nNFR{} of ``protecting patients privacy'' might create a conflict with ``patient claustrophobia'' requirement if the patients insist on keeping the curtains open while being dressed. 
It is important to identify these conflicts in the requirement elicitation stage.

% Restrictive
\boldparagraph{Restrictive \nNFRs}
Resolving conflicting requirements is challenging, it can lead to a too \emph{restrictive} set of \nNFRs{} that may not align with the goals of stakeholders. 
% example
For example, resolving conflicts between ``protecting patients' privacy'' and ``patient claustrophobia'' by mandating robots not to dress claustrophobic patients can be considered overly restrictive.
Striking the right balance is crucial in such situations. 
The resolution process should aim to address conflicts effectively without overly restricting the system's capabilities and its ability to achieve the initial goals.
It is therefore essential to maintain the focus on the system's primary objectives and ensure that the resolution does not compromise its functionality or intended purpose.

%Sufficient 
\boldparagraph{Sufficient \nNFRs}
\red{Alternatively, instead of ending up with too restrictive requirements, we may encounter a situation where we end up with normative requirements which are insufficient and fail to address the SLEEC concerns.
For instance, we might focus on addressing cultural and ethical concerns but inadvertently overlook the importance of addressing legal concerns.
It is crucial to determine whether the elicited requirements are \emph{sufficient} in addressing all relevant concerns.}
\hlTodo{TODO: add an example}

% Redundant requirements
\boldparagraph{Redundant requirements}
Different norms and factors can also share requirements, such as social and legal requirements often intersect by nature. 
% example
For example, a social requirement may state that the robot should respect the privacy of the patient, while a legal requirement may specify that the robot must adhere to relevant data protection laws and regulations. 
In such cases, the elicited requirement might be \emph{redundant}, which is not critical. 
\red{However, reducing unnecessary redundant requirements would simplify the validation and requirement reviewing process, and decrease the risk of inconsistency if one requirement is modified but the redundant one is not.}~\cite{Matsumoto-et-al-17}.

% Existing work
\boldparagraph{Existing work and the limitations}
When \red{validating} \nNFRs, prior research recommends using the SLEEC DSL, a state-of-the-art (SoTA) normative DSL, for specifying these requirements as \dsl{} rules~\cite{Getir-Yaman-et-al-23}.
For instance, some of the helper robot \nNFRs{} are expressed as \dsl rules in fig.~\ref{fig:examplefig}. 
Getir-Yaman et al.~\cite{Getir-Yaman-et-al-23} have proposed a technique based on model checking~\cite{Gibson-Robinson-et-al-14} to detect conflicts and redundancies among these rules. 
\red{Specifically, they identify if two rules exhibit conflicting responses when they share the same trigger.}
% example
For instance, consider the following two requirements: (r1)``When the patient requests to be dressed and the curtains are open, the robot must not dress the patient'' and (r2)``When the patient requests to be dressed, the robot must dress the patient within 2 minutes''. 
These requirements have conflicting responses given the same trigger, which is the ``patient's request to be dressed''.
\red{Similarly, Getir-Yaman et al. identify if two rules are redundant by examining rules that share the same trigger and intersect their responses.} 
% limitation
\red{Further validation of different conflict definitions is necessary to ensure a consistent set of rules.} 
\red{Existing preliminary work~\cite{feng-et-al-23-b} aattempted to identify conflicts and redundancies that arise given a trigger for all situations between multiple rules.
For example, let us consider the following three requirements: (r3) ``When the patient has fallen, call support'', (r4) ``When the patient has fallen, provide companionship to the patient'', and (r5) ``When you call support, leave the patient to not obstruct the space''. In this case, the requirement (r5) ``leave the patient when you call support'' conflicts with (r4) ``providing companionship'' when (r3) ``when you call support because the patient has fallen''.}
\red{However, other conflicts among \nNFRs{} remain not explored yet, specifically the ones occurring in specific situations. 
For instance, let us consider (r4') ``When the patient has fallen, provide companionship to the patient unless the patient is not deaf''. Here, the situation ``when the patient is deaf'' and the patient has fallen, a conflict arises.}
\red{This paper addresses the need to extend the identification of such conflicts.}

\boldparagraph{Conflicting, restrictive, sufficient, and redundant \nNFRs}
\hlTodo{TODO: remove the examples and instead refer to previous example, and name vacuous and situantional conflicts earlier.}
\red{In this paper, our focus is to further investigate whether a single \nNFR{} \emph{conflicts}, or is \emph{redundant}, with a set of \nNFRs. Furthermore, we also focus on studying whether a set of \nNFRs{} is too \emph{restrictive} to achieve the purpose of the system, and whether the set of \nNFRs{} is \emph{sufficient} to address the relevant SLEEC concerns.} 
%
\red{To further investigate whether a single rule conflicts with a set of rules, first,} we aim to determine if triggering the rule in any situation would lead to a violation of some other rule, resulting in a conflict. 
We refer to this as ``\emph{vacuous conflict}''. 
% example
For example, let's consider the two previous requirements (r1) and (r2) as an example of vacuous conflict. Indeed, triggering the patient's request to be dressed will lead to a violation in all situations. 
Additionally, we are interested in exploring whether a rule may interact with other rules in a contradictory manner, but only under specific situations.
These interactions can also lead to conflicts between different rules, which we refer to as ``\emph{situational conflict}''.
For instance, let's consider the following two requirements: (r6) ``When the patient requests to eat, feed the patient within one hour unless the patient must follow a specific diet, in which case, contact the doctor first'' and (r7) ``When the doctor is sleepy, do not contact the doctor for non-urgent matters''. \red{The two requirements are conflicting under the situation: the patient is hungry and must follow a specific diet, and the doctor is sleepy.}
%
To ensure that resolving \emph{vacuous} and \emph{situational} conflicts does not result in overly restrictive requirements, we propose to check whether the set of requirements is empty. 
In other words, we examine whether the intended purpose of the system can still be achieved given our \nNFRs. \red{Similarly, we can also check if the requirements are sufficient to exclude concerning behavior by checking the emptiness of their intersections.  }
%\green{NF: Emptiness check can also be used to determine if the concerns are sufficently blocked by the requirements. } \green{LM: If we add this, it can not be in restrictiveness, but we should add completeness, basically emptiness is the technique that we use to solve our problems, but what we solve is two different things, first whether the requirements are to restrictivie, and second whether the requirements are sufficient (so complete) to address the given concerns.}
%
Finally, we are interested in validating whether the resulting conflict-free rules are redundant with each other, as well as within themselves. 
Normative rules can be complex and composed of several defeaters, so we want to ensure that any redundant defeaters and rules are intentional.

% Contributions statement
\boldparagraph{Contributions} 
The paper makes three-fold contributions.
Firstly, it defines the identification of vacuous, situational-conflicting, restrictive, and redundant rules as satisfiability checking problems. Secondly, it proposes a formal tool called \tool that aids in the identification and diagnosis of these concerns when dealing with \nNFRs{} expressed as rules in the SoTA SLEEC DSL. 
\tool accomplishes this by translating the SLEEC DSL rules into \fol (first-order logic with quantifiers over relation object) and it utilizes the SoTA FOL* checker as a backend solver~\cite{feng-et-al-23}. 
Furthermore, \tool provides a non-technical diagnosis by highlighting the identified concerns within the input rules.
Finally, \tool includes a web interface~\cite{icse-tool}.
The artifact is available in~\cite{ICSE-Artifact}.


% Evaluation
\boldparagraph{Evaluation} 
\hlTodo{Add: sentence for the evaluation results.}


% Significance
\boldparagraph{Significance}
Checking \nNFRs{} for conflicts, restrictiveness, sufficiency, and redundancies in software engineering is essential for maintaining consistency %(e.g., conflicting requirements may lead to unpredictable or inconsistent outcomes)
, compliance% (e.g., proper resolution and adherence to applicable rules and regulations)
, efficiency% (e.g., redundant requirements can introduce unnecessary complexity and increase development and maintenance efforts)
, and risk mitigation% (e.g., addressing these issues proactively, software engineers can mitigate potential risks and enhance the overall quality and reliability of the software) 
in the development and maintenance of software systems. 
The diagnosis computed by \tool can be used by software engineers to (semi-)automatically generate and suggest patches to resolve redundancy, conflicts, and address concerns. 
The resulting conflict-free \nNFRs{} can be utilized by software engineers for designing and analyzing the system before deployment. 

% structure of the paper
The rest of this paper is organized as follows:
Sec.~\ref{sec:background} gives an overview of the SoTA normative \dsl and the \fol satisfiability checker. 
\hlTodo{TODO: agree on the structure of the paper and add it here.}
%Sec.~\ref{sec:specification} presents our extended domain-specific language, \dsle, and describes how it is translated into first-order logic with quantifiers over relational objects.
%Sec.~\ref{sec:redundancies-conflicts} provides definitions of redundant and conflicting rules.
%Sec.~\ref{sec:algo} describes the sanitization algorithm.
Sec.~\ref{sec:evaluation} presents the evaluation of the proposed approach's effectiveness.
Sec.~\ref{sec:conclusion} discusses  future research directions.  

%---------------------------------------------------------------------------------------------------------------
%-- Archive
%---------------------------------------------------------------------------------------------------------------

%\begin{itemize}
%    \item Start with non-functional requirements (RE, TSE, Empirical engineering, Workshops)
%    \item Defines qualities for these requirements
%    \item Check if expressible as \dsl rules (obligations which constraints only the future with continuous, or disjoints time windows.)
%    \item If not fully applicable, define subsets.
%    \item Goal: ``check if this is garbage''
%\end{itemize}

%\hl{Define normative requirements}

%\hl{Expressing the requirements as rules }

%\hl{Introduce the need of rules sanitization during and/or after the requirement elicitation process.} ~\cite{Lamsweerde-Darimont-Letier-98}

%\hl{Existing sanitization tool}

%\hl{Problem we solve in this paper}



==> Archive/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
% Context: normative requirements
Software systems interacting with humans are becoming prevalent in domains such as transportation~\cite{Pham-et-al-16,Nagatani-et-al-21}, and healthcare~\cite{Salceda-05,Laursen-et-al-22}, e.g., helper robots aimed to 
%% example
%For example, in healthcare~\cite{Salceda-05,Laursen-et-al-%22}, helper robots are being used to 
assist patients with dressing. 
The deployment of such systems raises significant concerns in the realms of social, legal, ethical, empathetic, and cultural aspects (referred to as SLEEC), e.g., \blue{a helper robot accidentally leaking a patient's private personal information when dressing them with the curtains open.} 
%that must be addressed during development~\cite{townsend-et-al-2022, Bremner2019DFW, Burton2020HMP}. 
% example
% For instance, to avoid that a dressing robot reveals a patient's personal information. 
%For instance, a helper robot might accidentally reveal patients' personal information without their consent.
To exclude such concerns effectively, 
researchers~\cite{townsend-et-al-2022, Bremner2019DFW, Burton2020HMP} proposed to use \emph{normative requirements}, i.e., non-functional requirements (NFRs) that restrict the acceptable range of system behavior.
%to exclude these concerns effectively.
%To tackle these concerns effectively, \emph{normative requirements} (\nNFRs) are defined, which are non-functional system requirements (NFRs) that restrict the acceptable range of system behavior to exclude the concerns. 
% example
For instance, \nNFRs{} for a helper robot may specify that the patient's well-being and privacy are prioritized by promptly completing the dressing task, especially when the patient is underdressed. 
\nNFRs{} are then used to inform all subsequent software engineering (SE) activities, such as design and validation. 

% SLEEC DSL
Prior research recommended using \dsl, a state-of-the-art (SoTA) domain-specific language~\cite{KOSAR201677}, for specifying \nNFRs{} as \dsl{} rules~\cite{Getir-Yaman-et-al-23,Getir-Yaman-et-al-23b}. \dsl{} is very close to natural language and has proven accessible to stakeholders without a technical background (e.g., lawyers, ethicists or regulators). A rule in \dsl{} can be accompanied by one or more \emph{defeaters}, introduced using the `\textbf{unless}' construct. Defeaters specify circumstances that preempt the original response and can optionally provide an alternative response. For instance, a simple normative rule $r1$ for a helper robot that supports dressing tasks for elderly individuals can be encoded as ``\textbf{when} DressingStarted \textbf{then} DressingCompleted \textbf{within} 3 minutes \textbf{unless} curtainsOpened \textbf{or} doorsOpened \textbf{then} Close \textbf{within} 2 minutes \textbf{unless} \textbf{not} personAssent''.

%It is therefore important to carefully elicit them, and to validate them at an early stage, to avoid the propagation of mistakes.

% NFRs challenges
\hlTodo{(Todo: Focus on complexity of N-NFRs, and tell that they need to be evaluated, we start with no-domain no-application specific validation, namely ...)}
Elicitation and early stage validation of non-functional requirements (NFRs) in general presents a complex, time-consuming process that is susceptible to errors~\cite{Meth-et-al-13,Didar-et-al-2005}. 
Typically, \blue{NFRs} can be specified by multiple stakeholders independently~\cite{Lamsweerde-Darimont-Letier-98}. 
These stakeholders have different concerns, priorities, and responsibilities.  Thus, \emph{well-formedness} issues such as \emph{conflicts}~\cite{Shah-et-al-21}, \emph{redundancies}, or \emph{insufficiencies}~\cite{Paech-et-al-04,Matsumoto-et-al-17,feng-et-al-23-b,Getir-Yaman-et-al-23} can arise during the elaboration of  NFRs, and support for addressing this has been proposed~\hlTodo{cite}.
% {\bf MC:  and now something about getting rid of conflicts}
Resolving conflicts is essential for ensuring the validity of NFRs whereby
identifying or removing  unnecessary redundant \blue{NFRs} simplifies the validation and reviewing process and decreases the risk of inconsistency if one \blue{NFR} is modified but the redundant one is not~\cite{Matsumoto-et-al-17}.
\blue{\red{It is also} important to ensure that the NFRs \red{is \textit{sufficiently} strong to address relevant concerns while} \red{is not overly} \emph{restrictive} to prevent system from achieving its initial objectives}.  {\bf MC: prev sentence does not parse} \green{\textbf{\underline{New}: is it better?}} 

% N-NFRs complexity 
\nNFRs{} present two additional layers of complexity.
 Firstly, the process includes challenges due to the involvement of stakeholders who often lack technical expertise.  While this problem is shared with NFRs in general, \nNFR{} stakeholders include experts with very different backgrounds:  lawyers, social workers, ethics experts, etc., and conflicting or redundant requirements can arise from different norms and factors~\cite{townsend-et-al-2022} even if elicited by a single stakeholder!
 Secondly, the task becomes even more complex when capturing intricate non-monotonic conditions expressed via \emph{if, then, unless} and time constraints (e.g., \textit{act within 1 week}), which are often abundant in \nNFRs~\cite{knoks2020,brunero2022,townsend-et-al-2022,feng-et-al-23-b}. 

% example
For example, consider a helper robot with the \nNFR{} of ``protecting patients' privacy'' ($r1$), which might \emph{conflict} with a ``patient claustrophobia'' \nNFR{} if the patient insists on keeping the curtains open while being dressed. Additionally, a social \nNFR{} may require respecting patient privacy, while a legal \nNFR{} may specify adherence to data protection laws, potentially creating a \emph{redundancy}. Resolving these issues may lead to \nNFRs{} that no longer align with stakeholder goals, either being overly \emph{restrictive} or \emph{insufficient} to address SLEEC concerns comprehensively.
%, such as overlooking important empathetic concerns, e.g.,  not providing empathetic communication to comfort the patient.}
% {\bf MC:  I do not follow.  I also feel that this paragraph can be much tigher} \green{\textbf{\underline{Simplified}}}

% Existing work
%\boldparagraph{Existing work on \nNFR{} \CRRI}
% intro SLEEC DSL
Existing work has analyzed certain \CRRI properties, such as redundancy and conflicts, but limited to interactions between only two \dsl rules~\cite{Getir-Yaman-et-al-23}, or ignoring specific contexts~\cite{feng-et-al-23-b}.
%as they do not consider larger rule sets or broader contexts, leading to missed errors – 
%as illustrated in the example below.
For instance, consider three \nNFRs{} expressed as \dsl rules: ($r2$) ``\textbf{when} PatientFallen \textbf{then} CallSupport'', ($r3$) ``\textbf{when} PatientFallen \textbf{then} provideCompanionship \textbf{unless} patientNotDeaf.'', and ($r4$) ``\textbf{when} CallSupport \textbf{then} not provideCompanionship''. In this case, the $r4$ (`do not provide companionship when you call support') conflicts with $r3$ (`providing companionship') in the situation where  `the deaf patient and has fallen' ($r2$). 
This conflict could not be detected using existing approach~\cite{feng-et-al-23-b}, but it represents a genuine threat to the validity of \nNFRs.
Existing approach~\cite{Getir-Yaman-et-al-23} also do not offer debugging assistance.
%In this context, by considering the full set of \nNFRs{} with broader context, we would identify be able to detect the conflict in the previous example. 

In this paper, we propose a comprehensive approach to analyze and debug \nNFRs{} \CRRI by checking a broad range of well-formedness constraints, including redundancy, conflicts (accounting for different contexts), restrictiveness, and insufficiency. 
To the best of our knowledge, our solution is the first to provide such an extensive analysis and debugging approach for \nNFRs.

%\boldparagraph{Conflicting, restrictive, insufficient, and redundant \nNFRs}
%{\bf MC:  intro needs to be rewritten from here on.}
%\boldparagraph{\nNFR{} \CRRI problem tackled in this paper}
%{\bf MC : this text screams "incremental work".  We are not further investigating.  We found an important problem that prior work did not solve and are now solving it.}
%In this paper, our focus is to further investigate whether a single \nNFR{} \emph{conflicts}, or is \emph{redundant}, with a set of \nNFRs. Furthermore, we also focus on studying whether a set of \nNFRs{} is too \emph{restrictive} to achieve the purpose of the system, and whether the set of \nNFRs{} is \emph{insufficient} to address the relevant SLEEC concerns.
%
%To further investigate whether a single rule conflicts with a set of rules, first, we aim to identify both \emph{vacuous} and \emph{situational} conflicts.  {\bf MC:  seems redundant with previous point.  In general, this paragraph and next are very long and do not help.  I propose to do this by example, followed by a short statement of contributions.}
%
%Then, we are interested in validating whether the resulting conflict-free rules are redundant with each other. %, as well as within themselves.\green{alcc: what does conflict within a rule means? } \green{\textbf{Answer}: It is not conflict, but redundancy within a rule, for instance if the defeaters are redundants (we observed this in our NIER evaluation).} 
%Normative rules can be complex, comprising several defeaters, so we want to ensure that any redundant defeaters and rules are intentional.
%
%To ensure that resolving \emph{vacuous}/\emph{situational} conflicts and \emph{redundancies} does not lead to excessively \emph{restrictive} requirements, we propose to check whether the set of requirements is too restrictive. %(i.e., the system main purposes are in the acceptable set of behaviours). 
%In other words, we examine whether the intended purpose of the system can still be achieved while adhering to our \nNFRs. 
%
%Finally, we check if the requirements are \emph{insufficient} in preventing concerning behavior.
%By checking whether there is any possibility for concerning behaviors to occur while still adhering to the \nNFRs. This helps us determine if our \nNFRs{} alone are sufficient to effectively prevent concerning behaviors.
%

% oveview schema
\input{Sections/Fig-latex/fig-approach}

% Contributions statement

\boldparagraph{Contributions}
This paper makes the following contributions: (a) a method for identifying  \CRRI issues in \nNFRs{} expressed in \dsl by converting them into satisfiability checking problems;
(b) a method for generating a non-technical diagnosis that pinpoints the causes of \CRRI issues by analyzing the causal proof of (un)satisfiability;
 (c) a validation of the effectiveness of the approach
 over 9 cases studies and 233 rules written by YYY non-technical and technical stakeholders.  
 %Technical and non-technical stakeholders collaborated in writing the normative requirements for each case study. 
% The stakeholders found \red{A}\% of the identified \CRRI issues to be relevant, and our diagnosis allowed them to resolve \red{B}\% of these issues. The artifacts are available at~\cite{ICSE-Artifact}.}
{\bf MC:  do not forget to mention, later, where the artifacts are available, and the tool.}
 
 Our approach, \approach, is implemented in a tool \tool -- see Fig.~\ref{fig:overview}.   \tool 
 %introduces \approach, a formal and tool-supported approach (depicted in Fig.~\ref{fig:overview})  to identify and diagnose  \CRRI issues in \nNFRs{} expressed in \dsl.\\
%\indent (B) By treating \CRRI issues as satisfiability checking problemsIt provides a tool for effective by treating them as satisfiability checking problems.}\\ 
\indent
%Specifically, \approach tackles \CRRI issue identification by formulating them as satisfiability checking problems.} \\
%\indent \blue{(B) \approach includes \tool, a tool that performs the following tasks:
%(B.1) Translating 
translates \nNFRs{} expressed as rules in the SoTA \dsl~\cite{Getir-Yaman-et-al-23,Getir-Yaman-et-al-23b} into first-order logic with quantifiers over relational objects (\fol)\cite{feng-et-al-23};
checks their satisfiability using the SoTA \fol{} checker~\cite{feng-et-al-23}; and generates a non-technical diagnosis. 
%
%(B.3) Generating a non-technical diagnosis that pinpoints the causes of \CRRI issues by analyzing the causal proof of (un)satisfiability.
%(B.4) Providing a web interface~\cite{icse-tool} for ease of use.} \\
%\indent \blue{(C) Collected nine real-world case studies, encompassing forest protection plans to deployed collaborative robots in the industry. In total, there are \red{$155$} \nNFRs{} evaluated to assess the effectiveness of \approach{} for identifying \CRRI issues and the usability of the diagnosis for resolving them. 


% Significance
\boldparagraph{Significance}
%Ensuring \CRRI of \nNFRs{} is essential for maintaining consistency, compliance,  efficiency, and risk mitigation  in the development and maintenance of software systems. The diagnosis computed by \approach can be used by software engineers to (semi-)automatically generate and suggest patches to resolve redundancy, conflicts, and address concerns. 
A comprehensive approach for analysis and debugging of \nNFRs{} is crucial in developing modern systems that increasingly interact with humans.  We believe that we are  the first to provide such an approach, supporting stakeholders with varying levels of technical expertise. Importantly, the diagnosis computed by \approach can be used by software engineers to (semi-)automatically generate and suggest patches for resolving issues, thereby further assisting the stakeholders with the \nNFR{} engineering  process.

% structure of the paper
The rest of this paper is organized as follows:
Sec.~\ref{sec:background} gives the background material for our work.
Sec.~\ref{sec:problem} defines the \nNFR{} \CRRI problem that we tackle in this paper.
Sec.~\ref{sec:sanitization} describes our approach, \approach, to identify \nNFRs{} \CRRI issues using \fol satisfiability checking.
Sec.~\ref{sec:diagnose} presents our approach that utilizes the causal proof of (un)satisfiability to highlight the reasons behind the \CRRI issues (e.g., conflict).
Sec.~\ref{sec:evaluation} presents the evaluation of the proposed approach's effectiveness.
Sec.~\ref{sec:relatedwork} compares \approach to existing NFR \CRRI checking approaches.
Sec.~\ref{sec:conclusion} discusses future research directions.
%---------------------------------------------------------------------------------------------------------------
%-- Archive
%---------------------------------------------------------------------------------------------------------------

%\begin{itemize}
%    \item Start with non-functional requirements (RE, TSE, Empirical engineering, Workshops)
%    \item Defines qualities for these requirements
%    \item Check if expressible as \dsl rules (obligations which constraints only the future with continuous, or disjoints time windows.)
%    \item If not fully applicable, define subsets.
%    \item Goal: ``check if this is garbage''
%\end{itemize}

%\hl{Define normative requirements}

%\hl{Expressing the requirements as rules }

%\hl{Introduce the need of rules sanitization during and/or after the requirement elicitation process.} ~\cite{Lamsweerde-Darimont-Letier-98}

%\hl{Existing sanitization tool}

%\hl{Problem we solve in this paper}

%Sec.~\ref{sec:specification} presents our extended domain-specific language, \dsle, and describes how it is translated into first-order logic with quantifiers over relational objects.
%Sec.~\ref{sec:redundancies-conflicts} provides definitions of redundant and conflicting rules.
%Sec.~\ref{sec:algo} describes the sanitization algorithm.

==> Archive/sanitization-archove.tex <==
\section{Sanitization with \fol Satisfiability} \label{sec:sanitization}

\red{\textbf{--------------------------------- COMING SOON ---------------------------------}}

\subsection{Encoding \dsl Rules in \fol}

\subsection{Inconsistencies Check via Satisfiability}


\red{\textbf{-------------------------------------------------------------------}}

\hlTodo{TODO: Introduce the} \approach, \hlTodo{in a header, 1) defining and encoding the identification of the} \nNFR{} \hlTodo{inconsistencies as satisfiability problem, 2) analyze UNSAT core to pinpoint the causes.}

% header
In this section, we present how to identify normative rules conflicts (vacuous and situational), redundancy, restrictiveness and sufficiency (see Sec.~\ref{sec:problem}) using \fol satisfiability checking.

\subsection{Restrictiveness/Insufficiency Check via Satisfiability}\label{sec:emptycheck}
%Given a set of rules and facts in $\dsl$, we can check if the behavior permitted by the rules contains all the facts (representing the desirable behaviors) via an emptiness check:

\red{Given a rule set $\ruleset$ and a set of facts representing some desirable (e.g., system purpose) or undesirable behaviors (e.g., SLEEC concerns), we can determine whether the behaviour permitted by the rules $\ruleset$ contains these facts via emptiness check:}

% It can determine whether the behaviour permitted by the rules contains all of the facts. It can also determine whether the set of rules is sufficient for excluding some undesirable behavior, also described as facts.

\begin{definition}[Rule Emptiness Check]\label{def:emptiness}
Let a rule set $\ruleset$ and a set of facts $\facts$ 
% {\bf MC:  does it matter what this represents?  aren't you just defining the emptyness check, without a particular intention?}
be given. 
 The emptiness check of   $\ruleset$ with respect to $\facts$ is
$\lang{\ruleset} \cap \lang{\facts} = \emptyset$.
\end{definition}

% It can determine whether the behaviour permitted by the rules contains all of the facts. It can also determine whether the set of rules is sufficient for excluding some undesirable behavior, also described as facts.

To check emptiness \red{(Def.~\ref{def:emptiness})} of $\ruleset$ with respect to $\facts$, we can check the satisfiability of the \fol constraint, $\translate{\ruleset} \wedge \translate{\facts}$, where $T$ is the  \fol translation function  defined in Tbl.~\ref{tab:translate}. \red{We first present the encoding function $T$ and then prove its correctness in Thm.~\ref{thm:transcorrectness}.}
% {\bf MC:  how does this connect with definition 11?}
% \red{\bf NF: we first presents the encoding function $T$, and then proves $T$ is correct in Thm.~\ref{thm:transcorrectness} where defintion 11 is used.}

\begin{figure*}
    \begin{tabular}{lll}
                \centering            $T(\rulesyntax{\event \wedge \prop}{\dobg})$ & \multicolumn{2}{l}{$\rightarrow$ $\forall \obj{\event}: \Class{\event}\exists \obj{\measures}:\Class{\measures}(\obj{\measure}.\textit{time} = \obj{\event}.\textit{time} \wedge (T^{*}(\prop, \obj{\measures}) \Rightarrow T^{*}(\dobg, \obj{\measures})))$}  \\
                
                $T(\factsyntax{\event \wedge \prop}{\dobg})$ & \multicolumn{2}{l}{ $\rightarrow$ $\exists \obj{\event}: \Class{\event}\exists \obj{\measures}:\Class{\measures}(\obj{\measure}.\textit{time} = \obj{\event}.\textit{time} \wedge (T^{*}(\prop, \obj{\measures}) \wedge T^{*}(\dobg, \obj{\measures})))$} \\
                
                $T^{*}(\cobg_1 \otherwise \cobg_2 \ldots \cobg_n, \; \obj{\measures})$& \multicolumn{2}{l}{$\rightarrow$ $T^{*}(\cobg_1, \obj{\measures}) \vee \exists \obj{\measures}_j:\Class{\measures}(\textbf{Violation}(\cobg_1, \obj{\measures}, \obj{\measures}_j) \wedge T^{*}(\cobg_2 \otherwise \ldots \cobg_n, \obj{\measures}_j))$} \\

                $T^{*}(\neg \dobg, \; \obj{\measures})$& \multicolumn{2}{l}{$\rightarrow$ $\neg T^{*}(\dobg)$} \\

                $T^{*}(\prop \Rightarrow \obg,  \obj{\measures})$&  \multicolumn{2}{l}{$\rightarrow$ $\neg T^{*}(\prop, \obj{\measures}) \wedge T^{*}(\obg, \obj{\measures})$} \\

                $\textbf{Violation}(\prop \Rightarrow \obg,  \obj{\measures}, \obj{\measures}_j)$&  \multicolumn{2}{l}{$\rightarrow$ $T^{*}(\prop, \obj{\measures}) \wedge \textbf{Violation}(\obg, \obj{\measures}, \obj{\measures}_j)$} \\
                
                $T^{*}(\within{\event}{\term},  \obj{\measures})$&  \multicolumn{2}{l}{$\rightarrow$ $\exists \obj{\event}:\Class{\event}(\obj{\measures}.\textit{time} \le \obj{\event}.\textit{time} \le \obj{\measures}.\textit{time} + T^{*}(\term, \obj{\measures}))$} \\

                $\textbf{violation}(\within{\event}{\term},  \obj{\measures}, \obj{\measures}_j)$&  \multicolumn{2}{l}{$\rightarrow$ $ \obj{\measures}_j.\textit{time} = \obj{\measures}.\textit{time} + T^{*}(\term, \obj{\measures})  \wedge \neg T^{*}(\within{\neg \event}{\term},  \obj{\measures})$ } \\

                $T^{*}(\within{\neg \event}{\term},  \obj{\measures})$& \multicolumn{2}{l}{ $\rightarrow$ $\neg T^{*}(\within{\neg \event}{\term},  \obj{\measures})$} \\

                $\textbf{Violation}(\within{\neg \event}{\term},  \obj{\measures}, \obj{\measures}_j)$&  \multicolumn{2}{l}{$\rightarrow$ \makecell{$ 
                (\obj{\measures}.\textit{time} \le \obj{\measures}_j.\textit{time} \le \obj{\measures}.\textit{time} + T^{*}(\term, \obj{\measures})) \wedge \exists \obj{\event}:\Class{\event}(\obj{\measures}_j.\textit{time} = \obj{\event}.\textit{time})$  \\ $\neg (\exists \obj{\event}_1:\Class{\event} (\obj{\measures}.\textit{time} \le \obj{\event}_1.\textit{time} < \obj{\measures}_j.\textit{time}) )$}} \\
                
                $T^{*}(c, \obj{\measures})$ $\rightarrow$ $c$  &  $T^{*}(\measure, \obj{\measures})$ $\rightarrow$ $\obj{\measures}.\measure$ &  \\
                $T^{*}(-\term, \obj{\measures})$ $\rightarrow$ $-T^{*}(\term, \obj{\measures})$& $T^{*}(\term_1 + \term_2, \obj{\measures})$ $\rightarrow$ $T^{*}(\term_1, \obj{\measures}) + T^{*}(\term_2, \obj{\measures})$ & $T^{*}(c \times \term, \obj{\measures})$ $\rightarrow$ $T^{*}(c, \obj{\measures}) \times T^{*}(\term, \obj{\measures})$\\
                
                $T^{*}(\top, \obj{\measures})$ $\rightarrow$  $\top$ & $T^{*}(\term_1 > \term_2, \obj{\measures})$ $\rightarrow$  $T^{*}( \term_1, \obj{\measures}) > T^{*}( \term_2, \obj{\measures})$ & $T^{*}(\term_1 = \term_2, \obj{\measures})$ $\rightarrow$  $T^{*}( \term_1, \obj{\measures}) = T^{*}( \term_2, \obj{\measures})$\\
                $T^{*}(\neg \prop, \obj{\measures})$ $\rightarrow$  $\neg T^{*}( \prop, \obj{\measures})$& $T^{*}( \prop_1 \wedge \prop_2, \obj{\measures})$ $\rightarrow$   $T^{*}( \prop_1, \obj{\measures}) \wedge T^{*}( \prop_2, \obj{\measures}) $ & $T^{*}( \prop_1 \vee \prop_2, \obj{\measures})$ $\rightarrow$   $T^{*}( \prop_1, \obj{\measures}) \vee T^{*}( \prop_2, \obj{\measures}) $
                \end{tabular}  
\caption{Translation rules from \dsl to \fol. Given a \dsl rule $\srule$, $T$ translates $\srule$ to an \fol formula using the translation function $T^{*}$. The function $T^{*}$ recursively visits the elements (i.e., term, proposition and obligations) 
% \hl{Discuss (we did not define components, should we say ``element'' instead, because component is a strong word)} 
of $\srule$ and translates them into \fol constraints under a relational object $\obj{\measures}$ representing the measures when $\srule$ is triggered. } 
\label{tab:translate}
\end{figure*}

\begin{figure*}
\begin{tabular}{| c | c | c |}
\hline
\makecell{ID} & \makecell{\dsl $\srule$} & \makecell{\fol $\translate{\srule}$}\\
\hline
$\srule_{c}$ &
 \makecell{$\textbf{when} \textit{OpenCurtainRqt} \; \wedge \; \neg \textit{underDressed}$  \\ $\textbf{then} \within{\textit{CurtainOpen}}{\textit{30 (sec)}}$} & 
 \makecell{$\forall \obj{cr}: \Class{\textit{OpenCurtainRqt}}\exists\obj{\measures}:\Class{\measures}$\\
    $(\obj{cr}.\textit{time} = \obj{\measures}.\textit{time} \wedge (\neg \obj{\measures}.\textit{underDressed} \Rightarrow$ \\ $\exists \obj{co}:\Class{\textit{CurtainOpen}} \obj{cr}.\textit{time} \le \obj{co}.\textit{time} \le \obj{cr}.\textit{time} + 30))$}\\
    \hline
    $\srule_{c'}$ &
 \makecell{$\textbf{when} \textit{OpenCurtainRqt} \; \wedge \; \neg \textit{underDressed}$  \\ $\textbf{then} \within{\textit{CurtainOpen}}{\textit{20 (sec)}}$} & 
 \makecell{$\forall \obj{cr}: \Class{\textit{OpenCurtainRqt}}\exists\obj{\measures}:\Class{\measures}$\\
    $(\obj{cr}.\textit{time} = \obj{\measures}.\textit{time} \wedge (\neg \obj{\measures}.\textit{underDressed} \Rightarrow$ \\ $\exists \obj{co}:\Class{\textit{CurtainOpen}} \obj{cr}.\textit{time} \le \obj{co}.\textit{time} \le \obj{cr}.\textit{time} + 20))$}\\
    \hline 
    $\fact_{c}$ & \makecell{$\textbf{exists} \textit{OpenCurtainRqt} \; \wedge \; \neg \textit{underDressed}$} &  
    \makecell{$\exists \obj{cr}: \Class{\textit{OpenCurtainRqt}}\exists\obj{\measures}:\Class{\measures}$\\
    $(\obj{cr}.\textit{time} = \obj{\measures}.\textit{time} \wedge \neg \obj{\measures}.\textit{underDressed})$}\\
    \hline
    $\violation{\srule_{c}}$ & \makecell{$\textbf{exists} \textit{OpenCurtainRqt} \; \wedge \; \neg \textit{underDressed}$ \\
    $\textbf{while} \within{\neg \textit{CurtainOpen}}{\textit{30 (sec)}}$} & \makecell{$\exists \obj{cr}: \Class{\textit{OpenCurtainRqt}}\exists\obj{\measures}:\Class{\measures}$\\
    $(\obj{cr}.\textit{time} = \obj{\measures}.\textit{time} \wedge (\neg \obj{\measures}.\textit{underDressed} \wedge$ \\ $\neg (\exists \obj{co}:\Class{\textit{CurtainOpen}} \obj{cr}.\textit{time} \le \obj{co}.\textit{time} \le \obj{cr}.\textit{time} + 30)))$} \\
    \hline
    $\srule_{c\times}$ & \makecell{$\textbf{when} \textit{OpenCurtainRqt} \; \wedge \; \neg \textit{underDressed}$ \\
    $\textbf{then} \within{\neg \textit{CurtainOpen}}{\textit{40}}$} & \makecell{$\forall \obj{cr}: \Class{\textit{OpenCurtainRqt}}\exists\obj{\measures}:\Class{\measures}$\\
    $(\obj{cr}.\textit{time} = \obj{\measures}.\textit{time} \wedge (\neg \obj{\measures}.\textit{underDressed} \Rightarrow$ \\ $\neg (\exists \obj{co}:\Class{\textit{CurtainOpen}} \obj{cr}.\textit{time} \le \obj{co}.\textit{time} \le \obj{cr}.\textit{time} + 40)))$} \\
    \hline
\end{tabular}





\caption{Examples of \hl{normalized} \dsl rules and their \fol translations. \hlTodo{TODO: Add an example with otherwise}}
\label{fig:examplefig}
\end{figure*}

To translate \dsl rules and facts into \fol constraints, the signature of \dsl is mapped to the signature of \fol as follows: (1) every event $\event \in \events$ is mapped to a class of  relational object $\Class{\event}$; and (2) every measure $\measure \in \measures$ is mapped to a named attribute in relational objects of class $\Class{\measures}$. \red{The function $T$ then translates every \dsl rule $\srule $ to a \fol formula $\translate{\srule}$ such that $\lang{\srule}$ is not empty if and only if $\translate{\srule}$ is satisfiable. $T$ follows the semantics of normalized $\dsl$ (Sec.~\ref{sec:background}). To translate the \textit{fulfillment} relation  with respect to a time point $i$ (i.e., $\models_i$), $T$ uses helper function $T^*$ to recursively visit element of the \dsl rule (i.e., obligations, propositions and terms) and encode the condition of fulfillment with respect to the time point $i$ (represented by the input relational object $\obj{\measures}$). $T$ also uses helper function \textbf{Violation} to translate the condition for obligations and conditional obligations to be violated at some time point $j$ (represented by the input relational object $\obj{\measures}_j$). }

More specifically, \red{$T$ translates a rule}
$\rulesyntax{\event \wedge \prop}{\dobg}$ to the following constraint: whenever the triggering event $\event$ occurs ($\forall \obj{\event}:\Class{event})$, the measures are available 
(i.e., $\exists \obj{\measures}:\Class{\measures}\cdot \obj{\event}.\textit{time} = \obj{\measures}.\textit{time}$), and if the measures 
 satisfy the triggering condition ($T^{*}(\prop, \obj{\measures})$), then the obligation chain is fulfilled ($T^{*}(\dobg, \obj{\measures})$). 
Similarly, every fact is translated to the constraint "there exists an occurrence of an event $\event$ ($\exists \obj{\event}:\Class{event})$, while the measures are available 
(i.e., $\exists \obj{\measures}:\Class{\measures}\cdot \obj{\event}.\textit{time} = \obj{\measures}.\textit{time}$) where the condition $\prop$ is satisfied ($T^{*}(\prop, \obj{\measures})$), and the obligation chain is  fulfilled ($T^{*}(\dobg, \obj{\measures})$)".
% \red{Notice that   
%  the function translation $T$ uses the helper function $T^*$, which recursively translates every element
% % \hl{\textbf{Discuss}: (same here, element?)}
% of the \dsl  rule (i.e., obligations, propositions and terms) under the \textit{current} measures represented by the relational object $\obj{\measures}$}. \hl{\textbf{MC:}  why now?}

To ensure that no two different measures for the same time point exist, we introduce the \fol \textit{measure consistency axiom}: $\textit{axiom}_{mc} \gets \forall \obj{\measures}_1, \obj{\measures}_2: \Class{\measures} (\obj{\measures}_1.\textit{time} = \obj{\measures}_2.\textit{time} \Rightarrow \obj{\measures}_1 \equiv \obj{\measures}_2)$, where $\equiv$ is the semantically equivalent relational constraint that asserts equivalence of every attribute between $\obj{\measures}_1$ and $\obj{\measures}_2$.

 \red{We now state and prove the correctness of the \fol encoding for emptiness checking:}


\begin{theorem}[Correctness of the \fol translation]\label{thm:transcorrectness}
Let a set of rules $\ruleset$ and facts $\facts$ in \dsl be given. There exists a trace $\fos = (\eventocc{1}, \measureassign{1}, \timestamp{1}),$ $ (\eventocc{2}, \measureassign{2}, \timestamp{2}),$ $\ldots  (\eventocc{n}, \measureassign{n}, \timestamp{n})$ such that $\fos \in \lang{\ruleset} \cap \lang{\facts}$ if and only if $\translate{\ruleset} \wedge \translate{\facts} \wedge \textit{axiom}_{mc}$ has a satisfying solution $(\domain, v)$.
\end{theorem}
% {\bf MC:  I am sorry, I do not follow.  How does this connect to the measure consistency axiom?  and why is it an axiom?}

\begin{sop}
    We prove the forward direction by constructing a satisfying solution $(\domain, v)$ to $\translate{\ruleset} \wedge \translate{\facts}$ from the trace $\fos \in \lang{\ruleset} \cap \lang{\facts}$. For every state $(\eventocc{i}, \measureassign{i}, \timestamp{i}) \in \fos$, we follow the construction rules: (1) for every event $\event \in \eventocc{i}$, add a relational object $\obj{e}$ of class $\Class{e}$ such that $v(\obj{e}.\textit{ext}) = \top$ and  $v(\obj{e}.\textit{time}) = \timestamp{i}$; and (2) add a relational object $\obj{\measures}$ such that $\obj{\measures}.\textit{time} = \timestamp{i}$ and $v(\obj{\measures}.m) = \measureassign{i}(\measure)$ for every measure $m \in \measures$. We then prove that the constructed $(\domain, v)$ is a solution to   $\translate{\ruleset} \wedge \translate{\facts} \wedge \textit{axiom}_{mc}$. 

    We prove the backward direction by constructing  $\fos$ from a satisfying solution $(\domain, v)$ to $\translate{\ruleset} \wedge \translate{\facts} \wedge \textit{axiom}_{mc}$. The construction maps every relational object $\obj{\event}$ and $\obj{\measures}$ to some state $(\eventocc{i}, \measureassign{i}, \timestamp{i}) \in \fos$, where (1) $\event \in \eventocc{i}$ if $v(\obj{\event}).\textit{ext} = \top \wedge v(\obj{\event}).\textit{time} = \timestamp{i}$; and (2) $\measureassign{\measure} = v(\obj{\measures}.\measure)$ for every $\measure \in \measures$ if $v(\obj{\measures}).\textit{ext} = \top \wedge v(\obj{\measures}).\textit{time} = \timestamp{i}$. We then prove $\fos \in \lang{\ruleset} \cap \lang{\facts}$ 
    and conclude the proof. 
    % {\bf MC:  do you mean that this shows that this proposition holds?}
\end{sop}



\begin{example}
    Consider the \dsl rule $\srule_{c}$ in Example~\ref{example:syntax}. The translated \fol constraint $\translate{\srule_{c}}$  is shown in Fig.~\ref{fig:examplefig}. The  $\dsl$ formalization of the fact "a user request to open the curtain while she is not under-dressed" and its translation into \fol are also shown in 
    %can be formalized  in $\dsl$ ($\fact_{c}$) and translated to \fol as shown in 
    Fig.~\ref{fig:examplefig}. The \fol formula $\translate{\srule_{c}} \wedge \translate{\fact_{c}}$ has a satisfying solution $(\domain, v)$ where (1) $\domain = \{\obj{\measures}_1, \obj{\measures}_2,$ $\obj{\textit{OpenCurtainRqt}}, \obj{\textit{OpenCurtain}}\}$; (2) $v(o.\textit{ext} = \top)$ for every $o \in \domain$; and (3) $v(\obj{\measures}_1.\textit{underDressed}) = \bot \wedge v(\obj{\measures}_1.\textit{time}) = 1$; 
    $v(\wedge v(\obj{\measures}_2.\textit{time}) = 2$. The solution is mapped to a trace $\fos = (\{\textit{OpenCurtainRqt}\}, \measureassign{1}, 1),$ $(\{\textit{OpenCurtain}\}, \measureassign{2}, 3)$ where $\measureassign{1}(\textit{underDressed}) = \bot$. \red{The trace $\fos$} is contained in $\lang{\srule_{c}} \cap \lang{\fact_{c}}$, and thus $\lang{\srule_{c}} \cap \lang{\fact_{c}}$ is not empty.  {\bf MC : so?}
\end{example}


\subsection{Detecting Redundancy via Satisfiability}
Recall from Def.~\ref{def:redudent}, a rule is redundant in a given rule set if and only if removing the rule from the rule set does not affect the behavior of the rule set.
By Def.~\ref{def:redudent}, 
%a rule $\srule \in \ruleset$
%is redundant if removing  the rule from $\ruleset$ does not change the %behavior of $\ruleset$. Therefore, 
$\srule$ is not redundant if and only if there exists a trace $\fos$ such that $\fos \models \ruleset \setminus \srule$ and $\fos \not\models \srule$. \red{ Fortunately, we are able to construct facts, refer as \textit{violations}, to describe the set of traces that violates a given rule. 
}

\begin{lemma}[Violations]\label{lemma:concern}
    Let a rule $\srule = \rulesyntax{\event \wedge \prop}{\dobg}$ be given. A trace $\fos \not\models \srule$ if and only if $\fos \models \violation{\srule}$ where  \red{$\violation{\srule}$ is the fact asserting the occurrence of $\event$ and a time where $\prop$ holds while violating $\dobg$} (\red{\quoted{$ \factsyntax{\event \wedge \prop}{\neg (\dobg})$}}).  
    {\bf MC:  I cannot parse this!}
\end{lemma}

\begin{example}
    A concern derived from a \dsl rule $\srule_{c}$ (Example~\ref{example:syntax},
    %from example~\ref{example:syntax}. The concern derived from $\srule_{c}$, 
    $\violation{\srule_c}$, is shown in Fig.~\ref{fig:examplefig}.
\end{example}

Lemma.~\ref{lemma:concern} enables detection of redundancy via satisfibility:

\begin{theorem}[Redundancy via Satisfiability]\label{Thm:redviasat}
    Let a set of \dsl rules ($\ruleset$) be given. A rule $\srule \in \ruleset$ is redundant if and only if $\translate{\ruleset \setminus \srule} \wedge \translate{\violation{\srule}} \wedge \textit{axiom}_{mc}$ is UNSAT. 
\end{theorem}

\begin{proof}
    By definition of redundancy (Def.~\ref{def:redudent}), $\srule$ is redundant if and only if there does not exist a $\fos$ such that $\fos \in \lang{\ruleset \setminus \srule}$ and $\fos \not\models \srule$. By Lemma~\ref{lemma:concern}, $\srule$ is redundant if and only if there does not exist a $\fos$ such that $\fos \in \lang{\ruleset \setminus \srule} \cap \lang{\violation{\srule}}$. By Thm.~\ref{thm:transcorrectness}, $\srule$ is redundant if and only if $\translate{\ruleset \setminus \srule} \wedge \translate{\violation{\srule}} \wedge \textit{axiom}_{mc}$ is UNSAT .
\end{proof}

\begin{example}\label{example:redudentSAT}
    Consider the rule set $\ruleset = \{\srule_{c}, \srule_{c'}\}$ in Example~\ref{exmaple:redudent}. The derived concern of $\srule_{c}$ and its \fol translation is shown in Fig.~\ref{fig:examplefig}. The \fol formula $\translate{\srule_{c'}} \wedge \translate{\violation{\srule_{c}}}$ is UNSAT, and thus $\srule_{c}$ is redundant in $\ruleset$.
\end{example}

Given a rule set $\ruleset$, we examine every rule in $\ruleset$ and check whether the rule is redundant by checking \fol satisfibility according to Thm.~\ref{Thm:redviasat}. In addition to reporting a binary "yes" or "no" answer, we also provide a diagnosis (if the rule is redundant), computed from a causal proof of UNSAT, to highlight the causes of the redundancy (see Sec.~\ref{sec:diagnose}).
%We will present the diagnose in Sec.~\ref{sec:diagnose}



\subsection{Detecting Vacuous Conflict via Satisfiability}\label{sec:conflictingchecking}
Recall from Def.~\ref{def:dconflict} that a rule $\srule \in \ruleset$ is vacuously conflicting in $\ruleset$ if the behavior defined by $\ruleset$ ($\lang{\ruleset}$)  trace where $\srule$ is triggered. In other words, triggering $\srule$ any situation will lead to a violation of some rules (and thus cause a conflict). Therefore, we can determine if a rule is vacuously conflicting by describing the set of traces where $\srule$ is triggered as facts in \dsl, and then checking whether it intersects with $\lang{\ruleset}$ via emptiness checking (Sec.~\ref{sec:emptycheck}). 

\begin{definition}[Triggering]\label{def:ruletrigger}
    Let a \dsl rule $\srule = \rulesyntax{\event \wedge \prop}{\dobg}$ be given. The \emph{triggering} of rule, denoted as $\triggerfunc{\srule}$, is the \dsl fact $\factsyntax{\event \wedge \prop}{\top}$.
\end{definition}

\begin{lemma}\label{lemma:vcdef}
    Let a set of rules $\ruleset$ be given. A rule $\srule \in \ruleset$ is vacuously conflicting if and only if $\lang{\ruleset} \cap \lang{\triggerfunc{\srule}}$ is empty.
\end{lemma}

Lemma~\ref{lemma:vcdef} is a direct consequence of Def.~\ref{def:dconflict} and Def.~\ref{def:ruletrigger}, and it enables vacuous conflict detection via satisfiability:

\begin{theorem}[Vacuous Conflict as Satisfiability]\label{thm:vcdef}
    Let a set of rules $\ruleset$ be given. A rule $\srule \in \ruleset$ is vacuously conflicting if and only if $\translate{\ruleset} \wedge \translate{\triggerfunc{\srule}} \wedge \textit{axiom}_{mc}$ is UNSAT.
\end{theorem}

\begin{proof}
    By Lemma~\ref{lemma:vcdef}, $\srule$ is vacuously conflicting if and only if $\lang{\ruleset} \cap \lang{\triggerfunc{\srule}}$ is empty. The emptiness checking problem can be encoded as the satisfiability problem by Thm.~\ref{thm:transcorrectness}.
\end{proof}

 \begin{example}
     Consider the rule set $\ruleset = \{\srule_{c} , \srule_{c\times}\}$ in Example~\ref{example:dconf}. The rules $\srule_{c}$ and $\srule_{c\times}$ and their \fol translations are shown in Fig.~\ref{fig:examplefig}. $\triggerfunc{\srule}$ is $\factsyntax{\textit{OpenCurtainRqt} \wedge \neg \textit{underDressed} }{\top}$. The \fol formula $\translate{\srule_{c}} \wedge \translate{\srule_{c\times}} \wedge \translate{\triggerfunc{\srule_{c}}} \wedge \textit{axiom}_{mc}$ is UNSAT, and thus $\srule_{c}$ is vacuously conflicting in $\ruleset$ due to $\srule_{c\times}$.
  \end{example}
    

Given a rule set, we examine each rule  to determine whether it is vacuously conflicting by checking \fol satisfiability using Thm.~\ref{thm:vcdef}. In addition to providing a binary "yes" or "no" answer, we also generate a diagnosis (in case the rule is redundant) obtained from a causal proof of UNSAT. This diagnosis helps highlight the causes of the conflict. The details of the diagnosis are in Sec.~\ref{sec:diagnose}.




==> Sections/evaluationOld.tex <==
\vspace{-0.1in}
\section{Evaluation}
\label{sec:evaluation}
% implementation

\vspace{-0.06in}
\noindent
\boldparagraph{Tool Support} We implemented our \approach approach in a tool \tool  (see the architecture in Fig.~\ref{fig:overview}). Input to \tool are \nNFRs{} expressed in \dsl.  Outputs are diagnoses for each \CRRI issue identified (e.g., Fig.~\ref{fig:unsatDiag}-\ref{fig:satDiag}). Built using Python, \tool encodes \dsl rules into \fol \CRRI satisfiability queries. It then uses \lego~\cite{feng-et-al-23} as the back-end to check \CRRI \fol satisfiability and produce the causal (un)satisfiability proof. Finally, it computes \CRRI diagnoses based on the proof. When no issues are identified, \tool produces a proof of correctness (i.e., absence of \CRRI). \tool also includes a user interface to
allow users to input \dsl rules.
%an encoder to encode the \CRRI checking problems into \fol satisfiability problem which could be solved by the back-end \fol satisfiability checker \lego.}
%\red{\tool c}
\tool together with the evaluation artifacts is available in \cite{ICSE-Artifact}.

%{\bf MC: Intro mentioned web support - do we describe it here as well?}
%\green{\underline{Answer}: We removed the web support}

%--- case-study table
%table
\begin{table}[t]
    \centering
    \sffamily
    \caption{{\small Case study statistics.}}
    \vspace{-0.1in}
    \scalebox{0.73}{
        \begin{tabular}{rcccccc}
        \toprule
            name & rules (evnt.$|$ msr.) &  defeaters & N-TS$|$TS & domain & stage \\\toprule
            ALMI & $39$ ($41|15$) &  $8$ & $2$ $|$ $2$ & social & deployed\\
             \cellcolor{gray!10}ASPEN & \cellcolor{gray!10} $15$ ($25|18$)& \cellcolor{gray!10}  $5$ & \cellcolor{gray!10} $2$ $|$ $2$ & \cellcolor{gray!10} env. & \cellcolor{gray!10} design\\
            AutoCar & 19 (36|26) &  20 & $1$ $|$ $1$ & transport & design\\
             \cellcolor{gray!10}BSN & \cellcolor{gray!10} 29 ($33$|$31$)& \cellcolor{gray!10}  $4$ & \cellcolor{gray!10} $2$ $|$ $2$ & \cellcolor{gray!10} health & \cellcolor{gray!10} proto.\\
            DressAssist & 31 (54|42) & 39 & $4$ $|$ $1$ & care & proto.\\
             \cellcolor{gray!10}CSI-Cobot & \cellcolor{gray!10} $20$ ($23$|$11$)& \cellcolor{gray!10}  $8$ & \cellcolor{gray!10} $2$ $|$ $1$ & \cellcolor{gray!10} manifacture & \cellcolor{gray!10} proto.\\
            DAISY & $26$ (45|31) &  20 & $3$ $|$ $1$ & health & proto.\\
             \cellcolor{gray!10}DPA & \cellcolor{gray!10} $26$ (28|25)& \cellcolor{gray!10}  $4$ & \cellcolor{gray!10} $1$ $|$ $1$ & \cellcolor{gray!10} education & \cellcolor{gray!10} design\\
            SafeSCAD & $28$ ($29$|$20$)&  $3$ & $2$ $|$ $1$ & transport & proto.\\
        \bottomrule
        \end{tabular}
    }
    \label{tab:caseStudyStats}  
    \vspace{-0.25in}
\end{table}
% add stage, domain, previous tool supported validation 


% header
We now evaluate the \emph{effectiveness} of \tool for identifying  \CRRI, and supporting a broad range of stakeholders in debugging them.
We ask the following research questions: 
How effective is  \tool in (\textbf{RQ1})  detecting \CRRI  and (\textbf{RQ2})  supporting debugging \CRRI?

\vspace{-0.03in}
% case-studies
\boldparagraph{Models and Methods}
We have divided the authors of the paper into two groups: the \emph{analysis experts} (AEs) who have defined and developed the approach, and the \emph{stakeholders}, further categorized into \emph{technical}  (TSs) and \emph{non-technical}  (N-TSs). We have ensured that there was no overlap between these groups. The stakeholders include: an ethicist, a lawyer, a philosopher, a psychologist, a safety analyst, and three engineers. The TSs identified nine real-world case studies from different stages, ranging from the design phase to deployed systems, as shown in Tbl.~\ref{tab:caseStudyStats}. 

The case studies were as follows. (1) ALMI~\cite{Hamilton-et-al-22}: a system assisting elderly and disabled users  in a monitoring or advisory role and with physical tasks; (2) ASPEN~\cite{aspen-23}: an autonomous agent dedicated to forest protection, providing both diagnosis and treatment of various tree pests and diseases; (3) AutoCar~\cite{autocar-20}: a system that implements emergency-vehicle priority awareness for autonomous vehicles; (4) BSN~\cite{Gil-et-al-21}: a healthcare system detecting emergencies by continuously monitoring the patient’s health status; (5) DressAssist~\cite{Jevtic-et-al-19,townsend-et-al-2022}: an assistive and supportive system used to dress and provide basic care for the elderly, children, and those with disabilities; (6) CSI-Cobot~\cite{Stefanakos-et-al-22}: a system ensuring the safe integration of industrial collaborative robot manipulators; (7) DAISY~\cite{daisy-22}: a sociotechnical AI-supported system that directs patients through an A\&E triage pathway; (8) DPA~\cite{Amaral-et-al-22}: a system to check the compliance of data processing agreements against the General Data Protection Regulation; (9) SafeSCAD~\cite{calinescu2021maintaining}: a driver attentiveness management system to support safe shared control of autonomous vehicles.
Case studies were chosen  (i) to test whether our approach scales with case studies involving complex \nNFRs{} with numerous defeaters and time constraints (AutoCar, DAISY, DressAssist); (ii) to examine the benefits of our approach on early-stage case studies (e.g., ASPEN and AutoCar), as compared to those at a more advanced stage (e.g., ALMI, DPA, BSN); (iii) to compare case studies involving many stakeholders (DressAssist, and DAISY) with those having fewer ones (DPA and AutoCar), and (iv) to consider different domains including the environment, healthcare, and transport.

For each case study, 1-2 TSs were paired with 1-4 N-TSs; together they built a set of normative requirements (\nNFRs). They then met to manually review, discuss, and agree on these \nNFRs. 
They specified a total of 233 \nNFRs. The number of \dsl rules ranged from 15 (ASPEN) to 39 (ALMI), and the number of defeaters in these rules ranged from 4 (DPA and BSN) to 39 (DressAssist).  Tbl.~\ref{tab:caseStudyStats} reports 
the number of events (evnt.), measures (msr.), rules (rules), defeaters (\textbf{unless}), and both technical (TS) and non-technical (N-TS) stakeholders  involved in the writing of the \nNFRs.

% table
\begin{table}[t]
    \centering
    \caption{\small  Run-time performance and  \CRRI. True positive (TP) and false negative (FP) issues identified for each  vacuous conflict (v-conf.), situational conflict (s-conf.), redundancy (redund.), restrictiveness (restrict.), and insufficiency (insuff.).  Spurious issues  are in bold.
    %Time and memory (mem) for identifying all the issues is also recorded.
    }
    \vspace{-0.1in}
    \scalebox{0.78}{
        \begin{tabular}{c c c c c c c}
             \toprule
            \multirow{ 2}{*}{case studies} & v-conf. & s-conf. & redund. & restrict. & insuffi. & time\\
            & (TP | FP) & (TP | FP) & (TP | FP) & (TP | FP) &  (TP | FP) & (sec.)\\ \toprule
           ALMI & 0 | 0 & 3| 0 & 0 | 0 & 0 | 0 &  1 | \textbf{1} & 30\\
            \cellcolor{gray!10} ASPEN &  \cellcolor{gray!10} 0 | 0 & \cellcolor{gray!10} 3 | 0 & \cellcolor{gray!10} 1 | 0 & \cellcolor{gray!10} 0 | 0 & \cellcolor{gray!10}  5 | 0 & \cellcolor{gray!10} 25.3\\
           AutoCar & 0 | 0 & 4 | 0 & 2 | 0 & 0 | 0 &  9 | 0 & 27.7\\
            \cellcolor{gray!10} BSN & \cellcolor{gray!10} 0 | 0 & \cellcolor{gray!10} 0 | 0 & \cellcolor{gray!10} 0 | 0 & \cellcolor{gray!10} 0 | 0 & \cellcolor{gray!10}  3 | 0 & \cellcolor{gray!10} 46\\
           DressAssist & 0 | 0 & 1 | 0 & 0 | 0 & 0 | 0 &  1 | \textbf{3} & 20.3\\
            \cellcolor{gray!10} CSI-Cobot & \cellcolor{gray!10} 0 | 0 & \cellcolor{gray!10} 0 | 0 & \cellcolor{gray!10} 2 | 0 & \cellcolor{gray!10} 0 | 0 & \cellcolor{gray!10} 6 | \textbf{1} & \cellcolor{gray!10} 25.3\\ 
           DAISY & 0 | 0 & 1 | 0 & 1 | 0 & 0 | 0 &  5 | 0 & 30.4\\
            \cellcolor{gray!10}DPA & \cellcolor{gray!10}  0| 0  & \cellcolor{gray!10} 0| 0 & \cellcolor{gray!10} 0 | 0 & \cellcolor{gray!10} 0 | 0 & \cellcolor{gray!10} 4 | 0  & \cellcolor{gray!10} 21.4\\
           SafeSCAD & 0 | 0 & 8 | 0 & 2 | 0 & \textbf{2} | 0 & 4 | \textbf{1} & 42.4\\
           \bottomrule
        \end{tabular}
    }
    \label{tab:identifyIssues}
    \vspace{-0.2in}
\end{table}


% total- reoslution effort - too complex
\begin{table}[t]
    \centering
    \caption{\small Effectiveness of \tool for supporting debugging of non-spurious \CRRI  in Tbl.~\ref{tab:identifyIssues}. Metrics are: \# of issues, \# of added events or measures (add D), \# of added  (add R), refined, merged, and deleted rules, and \# cases classified as too complex.} 

    \vspace{-0.1in}
    \scalebox{0.78}{
        \begin{tabular}{ccccccccc}
        \toprule
             %\multirow{ 2}{*}{case studies} & \multicolumn{2} {c} {diagnosis helpful}  \\
             \multirow{ 2}{*}{case studies} & \multirow{ 2}{*}{total} &  \multicolumn{5} {c} {resolution effort} & \multirow{2}{*}{complex} \\
              &  & add D & add R & refine & merge & delete &  \\  \toprule
             ALMI & $4$ &  1& 4 & 0 & 0 & 1 & - \\ 
              \cellcolor{gray!10} ASPEN &  \cellcolor{gray!10} $9$  & \cellcolor{gray!10} 1 & \cellcolor{gray!10} 3 & \cellcolor{gray!10} 3 & \cellcolor{gray!10} 1 & \cellcolor{gray!10} 2  &  \cellcolor{gray!10}  - \\ 
             AutoCar & 11 & 1 & 20 & 4 & 0 & 1 & - \\ 
              \cellcolor{gray!10} BSN &  \cellcolor{gray!10} 3 & \cellcolor{gray!10} 3 & \cellcolor{gray!10} 3 & \cellcolor{gray!10} 0 & \cellcolor{gray!10} 0 & \cellcolor{gray!10}0  &  \cellcolor{gray!10}  - \\
             DressAssist & $1$ & 1 & 0 & 1 & 0 & 0 & - \\
              \cellcolor{gray!10} CSI-Cobot &  \cellcolor{gray!10} $8$ & \cellcolor{gray!10} 3 & \cellcolor{gray!10}7 & \cellcolor{gray!10} 1 & \cellcolor{gray!10}0 & \cellcolor{gray!10}1 &  \cellcolor{gray!10}  - \\ 
             DAISY & $7$ & 0 & 5 & 1 & 1 & 0 & - \\ 
              \cellcolor{gray!10} DPA &  \cellcolor{gray!10} $4$ & \cellcolor{gray!10}0 & \cellcolor{gray!10} 4 & \cellcolor{gray!10}1 & \cellcolor{gray!10}0 & \cellcolor{gray!10} 2 &  \cellcolor{gray!10}  - \\ 
             SafeSCAD & $16$ & 5 & 6 &  9 & 4 & 2 & \textbf{1} \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:diagnosishelpful}
    \vspace{-0.25in}
\end{table}
% understanding (U/N) - resolving (yes/no) - resolved (yes/time/complex) - complex resolution - 

\vspace{-0.03in}
\boldparagraph{RQ1}
Once the  \nNFRs{} were built,
the AEs met with the TSs and N-TSs involved in each case study to evaluate the \CRRI, in one session for each case study. 
When no issue was identified, AEs provided a proof of correctness. We focused on the stakeholders' ability to understand the feedback given by \tool and split the identified concerns into \emph{relevant} (TP) or \emph{spurious} (FP). Additionally, the stakeholders specified which part of the diagnosis helped them understand and perform this classification. The results are in Tbl.~\ref{tab:identifyIssues}.  

%of the case study \nNFRs  (i.e., nine sessions).}  
It took \tool between 21 and 49 seconds to analyze the \nNFR{} \CRRI in each case study, using a ThinkPad X1 Carbon with an Intel Core i7 1.80 GHz processor, 8 GB of RAM, and running 64-bit Ubuntu GNU/Linux 8. 
%
% Vacuous conflicts
No vacuous conflicts were identified, likely
 due to the careful manual review of the rules prior to our analysis. To ensure correctness, we augmented the proof of absence of vacuous conflicts produced by \tool with
feedback produced by AutoCheck~\cite{feng-et-al-23}, an existing tool for analyzing vacuous conflicts. This evaluation, see \cite{ICSE-Artifact}, confirmed the soundness of our approach.
%w.r.t. the identification of vacuous conflicts. 

% Situational conflicts
\tool identified 20 situational conflicts involving each 2-3  rules, and highlighted 2-3 environment constraints from the 20 to 33 possible ones.   This means that the rules conflict only in highly limited environments.
%This means that there are rules conflicting only in specific situations (specific environment).
Reviewing these conflicts without tool support is quite challenging, especially for case studies involving many rules (DAISY) or numerous environmental constraints  (e.g., DAISY, AutoCar, and ASPEN). 
Here, the diagnosis helped stakeholders  understand the issue by: (1) specifying which rules to focus on; (2) pinpointing the specific clauses causing the conflicts;  and (3) providing a trace specifying the situations in which the conflicts occur and the blocked response, thus aiding stakeholders in understanding the environments under which the conflicts occur.
%under which environments the conflicts occur.
% Redundancy
\tool also identified eight redundancies involving 2-3 rules each.  The diagnosis provided all the necessary information to understand each redundancy, including identifying and extracting redundant rules and highlighting  redundant clauses. Stakeholders quickly confirmed that none of these redundancies were intentional, so
the identified redundancies were unnecessary and could have led to future inconsistencies.
% Purpose
Regarding restrictiveness, one case study, SafeSCADE, was found to have \nNFRs{} that were too restrictive, preventing the system from achieving two of its main purposes. 
%Specifically, for each purpose, one rule with the environment and time constraints was preventing the system from fulfilling these purposes. 
The provided diagnosis directly helped the stakeholders.
%understand the reasons.% for that.
%why the rule was too restrictive.

% Concerns
Cases of insufficiency were identified in every case study, raising the total of 38 concerns. 
%also reported six spurious concerns. 
%Classifying the concerns as spurious or relevant was not a trivial task. 
Determining the spuriousness of some concerns required a non-trivial  examination and consideration process.
Specifically, the stakeholders analyzed the traces provided by our diagnosis (e.g., Fig.~\ref{fig:unsatDiag}) and engaged in detailed discussions on whether their rules needed to address each identified concern, e.g., whether enabling patients to disconnect sensors tracking their health is a bad behaviour.
At the end, they identified spurious concerns only in four case studies.
%At the end, they limited spurious only to ALMI, CSI-Robot, DressAssist, and SafeSCADE.
% they identified spurious concerns only in
%Many factors could cause the spuriousness. 
%For instance, spurious concerns in the DressAssist case study resulted from an imprecise specification regarding the consideration of defeaters (notably, DressAssist had the highest number, 39, of defeaters among all nine case studies).
%Similarly, the spurious concerns in the CSI case study were due to inconsistent specifications.
%Finally, in SafeSCADE, the spurious concern also arose from an imprecise specification of not considering the priority. Although spurious, the stakeholders decided to refine the definitions to make the priority explicit. 
%Overall, 100\% of situational conflicts, 100\% of redundant rules, 100\% restricted system purposes, and \red{84\%} of the raised concerns identified by \tool were determined by the stakeholders to be relevant.
The feedback provided by \tool enabled the stakeholders to understand the meaning of the identified cases for all types of \CRRI, limiting spurious feedback to raised concerns. Thus, we successfully answered RQ1.
% "we established effectiveness of our approach (RQ1)
% Thus, we successfully answered RQ1.


\vspace{-0.05in}
\boldparagraph{RQ2}
%We intend to use these case studies to measure the number of spurious \CRRI issues that \tool identifies. We will do this by presenting them to the stakeholders and asking whether they are relevant. 
%We aim to answer the following question: 
% intro Q2
%Secondly, we evaluate the usability of \tool's \CRRI diagnosis in aiding stakeholders to resolve the \CRRI issues. 
Once the stakeholders understood and classified each identified \CRRI issue as non-spurious, we asked them, in the same session, to use the diagnosis to \emph{debug} the issue.  We recorded the resolution effort, i.e., the number of definitions/rules added, refined, merged or deleted, as a proxy to the resolution complexity. 
The results are in Tbl.~\ref{tab:diagnosishelpful}. 
% redundancy
The enumeration of redundant rules along with the highlighting of redundant clauses (e.g., Fig.~\ref{fig:unsatDiag}) provided by \tool enabled the stakeholders to easily resolve the cases of redundancy. They knew directly what to fix (mostly merge, delete, or refine).
%thanks to the clear identification provided by the diagnosis.
% situational conflicts
\tool supported the stakeholders in resolving situational conflicts by:
(1) specifying the specific clauses causing the conflicts, which enabled stakeholders to focus on these rules, making the resolution process more targeted;
(2) providing the event and measure values representing the situations in which the conflicts occurred, which helped stakeholders consider the environmental constraints comprehensively while devising a resolution strategy (merging and refining both rules and definitions),
and (3) highlighting the blocked response in  the trace  (e.g., see Fig.~\ref{fig:unsatDiag}), which allowed stakeholders  study priority between the conflicting rule responses.
%Resolving situation conflict, resulted in merging and refining both rules and definitions
%Last, a single rule was refined multiple times for this case study (as well as for ASPEN), and resolving situational conflicts helped the stakeholders to be comprehensive in terms of considering the environmental constraints.

% insufficiency
Regarding insufficiency, the stakeholders specifically appreciated the optimal size of the trace (e.g., Fig.~\ref{fig:unsatDiag}), as it helped them understand which events interfere with the identified concerns.
%However, all of them agreed that having hints about the patching type (refine or add) and, if refining, which rule must be refined,
% would have saved them time.  
%This is because resolving insufficiency mostly involved the stakeholders in refining existing rules (adding some constraints or defeaters) or adding a new rule to address the raised concern.
% restrictiveness
Regarding restrictiveness, the tool  provided all of the necessary information (i.e., pinpointed clauses on the rules restricting the system purpose) for the stakeholders to straightforwardly and trivially resolve the issue. Resolving restrictiveness issues (only two instances found across all the case studies) resulted in refining and merging the rules. 
In the case of AutoCar, checking restrictiveness helped refine constraints and correct incorrect responses, as well as establish priority between the rules, ultimately simplifying the rules.   
It also enabled the refinement of definitions and rules to be more specific (less restrictive), 
i.e., by introducing an additional event {\small\texttt{StopAutonomousAssistance}} instead of {\small\texttt{CarDriving}} for the rule \textbf{when} {\small\texttt{DisplayError}} \textbf{then} {\small\texttt{StopAutonomousAssistance}}.
%

For the majority of resolutions, stakeholders added a rule (60\%) or refined an existing one (23\%). They very rarely removed one (10\%), and even less frequently merged existing rules (7\%).
Our diagnosis supported the stakeholders  in resolving the \CRRI  when time allowed.  
Therefore, we successfully answer RQ2.

\vspace{-0.03in}
\boldparagraph{Summary}
Our experiment demonstrated that our approach effectively and efficiently identifies \nNFR{} \CRRI. 
Both technical and non-technical stakeholders found the diagnosis to be comprehensible and helpful in resolving the identified issues. 
Notably, \tool allowed stakeholders to add missing rules and encouraged them to consider missing cases without constraining their imagination during the elicitation process. 
The inclusion of traces proved beneficial for stakeholders, enabling them to understand concerns that were not addressed by their \nNFRs{} and providing insights into the situations where conflicts occurred. 
However, stakeholders expressed the desire for a methodology to aid in issue resolution, as well as suggestions for potential resolution patches. They also would have preferred
%Additionally, stakeholders mentioned thatthey would have appreciated 
using the tool during the elicitation process to help them identify and address potential issues proactively. Overall, the stakeholders really appreciated the assistance provided by \tool in addressing the \CRRI.

\vspace{-0.03in}
\boldparagraph{Threats to validity}
(1) 
The case studies were built by the co-authors of this paper. We mitigated this threat by separating the authors onto those who developed the validation approach and those who built the case studies, and ensured that a complete separation between them was maintained throughout the entire lifecycle of the project.
(2)
While we considered only nine case studies,  we  mitigated this treat by choosing them from different domains, at different development stages, and written by stakeholders with different types of expertise. Developing, collecting, evaluating these case studies took around
140 hours of work, resulting, to the best of our knowledge, in the most extensive collection of normative requirements to date.
%resulted in approximately a total of \red{169} hours of work. 
%We are not aware of an existing normative requirement benchmark as extensive as ours.\\
%
(3)
The number of identified issues was relatively modest  because we 
% \red{allow unlimited amount of time for the stakeholders to manually analyze and refine the requirements before commencing the experiments.}
started with existing systems where many issues had already been resolved, and followed the stakeholders' manual analysis.
%a `realistic' set of \nNFRs{}, where many issues had already been resolved by stakeholders' manual analysis (with unlimited amount of time) during their design). }
%{\bf MC: 
% prev sentence is ugly.}
% The stakeholders also reviewed their \nNFRs{} before the analysis commenced.  
Yet the stakeholders mentioned that they would have preferred to bypass this manual reviewing meeting and use our tool directly, as it would have saved them at least 10 hours. %between all the case studies.

%---------------- Archive

% Feedback
% participant would ave preferde, no manual evaluation but direct evaluation wih the tool
% Diagnosis helpful, stakholder would appeciate to use the tool iteratively while eliciting the rules
% Extra fetaure provide a hint on repair, maybe at least type: refine/ add/ merge rules
% Future work and stakeholder feedback, need for defining a process for systematically specifying concerns. This can be complex when the concerns are heavily dependent on the environment, a situation often identified by the defeaters
% Diagnosis feedbcak
% ....
% overwelhing to get all the outputs at once. 
% positive feedback on the diagnosis to understand the problems in the requirements and understand stakehodlers's each other. 
% they require mapping, corresponding rules in natural language when any problem is arised. 

% they would have liked to have the tool earlier.



% build a case-study by co-authos not involved in the anaysis, or 
% order of properties verification, and 
% not asking enough question, not representive stakeholders or case studies, only 9, tell how much time. We mitigate this by explicitle icling a range of examples and states, from different domains, and a broad range of expert. (enough questions to enough people)
% spurious concerns specification
% (construct, test), complexity rules,  
% depend on correct specification of concerns, and purpose. 
% rely on expert jugement, mitigate recording their reasoning, asking them to explain us the reason (internal).
% 


%---------------- Archive
%[Construct] % does the test measure the content?
%[Internal] % order of properties verification,   (given what you did, did you obeserve what you did) (did you measure right) (methodology)
% mitigated resolution with multiple mitigation (given input do I observe output)
%[External] % not asking enough question, not representive stakeholders or case studies, only 9, tell how much time. We mitigate this by explicitle icling a range of examples and states, from different domains, and a broad range of expert.
% spurious concerns specification
% generailizarion
% what they said it is not what they think they said

==> Sections/redundancies-conflicts.tex <==
\section{UNSAT-proof based Diagnose}
\label{sec:diagnose}

\hl{TODO: definitions of conflicts, redudancy (within the rule as well), and examples.}

==> Sections/response.tex <==
\setcounter{page}{1}
\renewcommand{\thepage}{\roman{page}}

\section*{Responses to the Reviewers}
We are grateful to the reviewers for their thorough examination of our work and their relevant remarks. We carefully considered the required changes and updated the text accordingly. We hope that upon acceptance, we will have the opportunity to address additional suggested changes that were not mandatory for this revision, after being able to use an additional page.  In the revised submission, the newly added text is indicated in \blue{blue}. All required changes are listed below (in \red{red}), together with our responses (in black).

\noindent
\textbf{Required changes for papers recommended for revision:}

\begin{itemize}
    \item \red{1. RQ2 was not investigated systematically and appears more like an exploratory study on how stakeholders used the tool to improve the quality of the requirements. The authors should remove RQ2 and frame its content in a discussion section.}

[Response:]
In compliance with the requested changes, we have removed RQ2 from Section~\ref{sec:evaluation}. The content previously under this research question has been restructured and is now presented in the form of a discussion, which precedes the summary of the evaluation.

    \item \red{2. Because the stakeholders who developed the requirements specification were also asked to evaluate the usefulness of the diagnostic technique, they may be biased in the evaluation of the usefulness of the technique. The authors need to discuss this threat to validity in the paper.}

[Response:] In Section~\ref{sec:evaluation}, we discuss this treat of validity and further explain our rationale for using the same stakeholders for both collecting requirements and validating our tool.

    \item \red{3. Include a more compelling motivation to justify using FOL* as the underlying formalism for SLEEC.}

[Response:] 
We have incorporated an additional paragraph in the Introduction to elucidate the motivation behind utilizing FOL* as the underlying formalism for SLEEC. This clarification appears just before we outline the contributions of this paper.


\end{itemize}



==> Sections/specification.tex <==
\section{Specification}
\label{sec:specification}

\boldparagraph{Syntax}
A \dsle signature is a tuple $(C, E, M, \iota, \gamma)$. $E$ is set predicate symbol for event, and  $C$ , $M$ are function symbols for constants and measures, respectively.  
The function $\iota: (C \cup E \cup M ) \rightarrow \mathbb{N}$ associate every function (and predicate) with an arity.  
Function $\gamma: (C \cup M) \rightarrow \{\mathbb{Z}, \mathbb{B}\}$ associate each function's output with a datatype. 
For simplifying the presentation, we assume \dsle supports only integer ($\mathbb{N}$) and boolean ($\mathbb{B}$) while scalars can be interpreted as integers under constraints. 
Using $\gamma$, we partition $M$ into $M^b$ and $M^i$ for the set of measure symbols with type $\mathbb{B}$ and $\mathbb{Z}$ respectively. Similarly, we partition $C$ into $C^b$ and $C^i$ based on constants' data type. 

Let \dsle signature $(C, E, M, \iota, \gamma)$ be given. Boolean ($t^b)$ and integer ($t^i)$, inductively as:
% following grammar rule (5-10) shown in Table~\ref{tab:sleec-gram}. \red{TODO: continue}
A \dsl rule (3) has the syntax \sleeckeyword{when} \textit{trigger} \sleeckeyword{then}  \textit{response}. The \textit{trigger} (4) of a rule is always an event symbol $e \in E$ with a Boolean term representing the condition. A \textit{response} (15) of a rule is the presence / absence of an event (\textit{occ}) followed by \textit{alternative} and \textit{defeaters}. 
The syntax of \textit{occ} (17), \textit{alternatives}(18) and \textit{defeaters} (19) is shown in~\ref{tab:sleecplus-gram}. 
Defeaters is a sequence of defeater, where each defeater has a Boolean term as its condition and a \textit{response} as its consequence. Defeaters can be nested since a defeater's response can have its own defeater. However, the maximum level of nesting must be finite (i.e., without recursive defeaters). A ruleset $R$ is a set of \dsle rules. 


\begin{table}[t]
    \centering
    \scalebox{0.65}{
        \begin{tabular}{l c l}
        \toprule
            specification &    & defBlock ruleBlock\\\toprule
            defBlock &   & \sleeckeyword{def\_start} definitions \sleeckeyword{def\_end}\\
            definitions &    & definition $|$ definition definitions\\
            definition &    & event $|$ measure $|$ constant\\
            event &   & \sleeckeyword{event} eventID \hln{[{\sleeckeyword{(}}parameters{\sleeckeyword{)}}]}\\
            \hln{parameters} &  & \hln{parameter $|$ parameter parameters}\\
            \hln{parameter} &  & \hln{boolParameter $|$ numParameter $|$ scalarParameter}\\
            \hln{boolParameter} &  & \hln{boolParamID: {\sleeckeyword{boolean}}}\\
            \hln{numParameter} &  & \hln{numParamID:} \underline{{\sleeckeyword{numeric}}}\\
            \hln{scalarParameter} &  & \hln{scalarParamID: scale} \\
            measure &   & boolMeasure $|$ numMeasure $|$ scalarMeasure \\
            boolMeasure &   & \sleeckeyword{measure} boolMeasureID \hln{[{\sleeckeyword{(}} parameters {\sleeckeyword{)}}]}: \sleeckeyword{boolean}\\
            numMeasure &   & \sleeckeyword{measure} measureID \hln{[{\sleeckeyword{(}}parameters{\sleeckeyword{)}}]}: \sleeckeyword{numeric}\\
            scalarMeasure &   & \sleeckeyword{measure} measureID \hln{[{\sleeckeyword{(}}parameters{\sleeckeyword{)}}]}: scale\\
            constant &   & \sleeckeyword{constant} constID [=value]\\
            %type &  ::= & \sleeckeyword{boolean} $|$ \sleeckeyword{numeric} $|$ scale\\
            scale &   & \sleeckeyword{scale} \sleeckeyword{(}scaleArgs\sleeckeyword{)}\\
            scaleArgs &    &  argID $|$ argID, scaleArgs\\\toprule
            ruleBlock &    & \sleeckeyword{rule\_start} rules \sleeckeyword{rule\_end}\\
            rules &    & rule $|$ rule rules\\
            rule &    & ruleID \sleeckeyword{when} trigger \sleeckeyword{then} response\\
            trigger &    & eventID \hln{[{\sleeckeyword{(}} bindings{\sleeckeyword{)}}]} $|$ eventID \hln{[{\sleeckeyword{(}} bindings{\sleeckeyword{)}}]} \sleeckeyword{and} boolExpr\\
            \hln{bindings} &  & \hln{binding $|$ binding bindings} \\
            \hln{binding} &  & \hln{boolParamID {\sleeckeyword{=}} boolParamValue} $|$ \hln{numParamID {\sleeckeyword{=}} numParamValue} $|$ \\
            &&\hln{scalarParamID {\sleeckeyword{=}} scalarParamValue}\\
            \hln{boolParamValue} &  & \hln{boolParamValueID $|$ boolExpr}\\
            \hln{numParamValue} & & \hln{numParamValueID $|$ numExpr} \\
            \hln{scalarParamValue} & & \hln{scalarParamValueID $|$ scalarTerminal}\\
            boolExpr & & boolTerminal $|$ negation $|$ binaryExpr \hln{$|$ quantificationE}\\
            \hln{quantificationE} & & \hln{{\sleeckeyword{(some}} eventID {\sleeckeyword{(}}bindings{\sleeckeyword{)}} {\sleeckeyword{where}} boolExpr{\sleeckeyword{)}}} %\hl{TODO:semantic}
            \\
            boolTerminal &  & \sleeckeyword{true} $|$  \sleeckeyword{false} $|$ boolMeasureID \hln{$|$ boolParamValueID} %\hl{TODO: add semantic constraint} 
            \\
            negation &  & \sleeckeyword{(not} boolExpr\sleeckeyword{)}\\
            binaryExpr &  & boolBinaryExpr $|$ numericBinaryExpr $|$ scaleBinaryExpr\\
            boolBinaryExpr & & boolExpr boolOp boolExpr\\   
            numericBinaryExpr & & numExpr relOp numExpr \\
            scaleBinaryExpr & & scaleTerminal relOp scalaTerminal \\
            numExpr & & numericTerminal $|$ numBinFunc \\
            numericTerminal & & value $|$ numMeasureID \hln{$|$ numParamValueID}\\
            numBinFunc & & numExpr numOp numExpr \\
            scaleTerminal & & argID $|$ scaleMeasureID \hln{$|$ scalarParamValueID}\\
            response &   & occ [alternative] [defeaters] $|$ \sleeckeyword{\{}occ [alternative] [defeaters]\sleeckeyword{\}} \\
            occ &    & [\sleeckeyword{not}] eventID [\sleeckeyword{within} value timeUnit] \\
            alternative &     &  \sleeckeyword{otherwise} response \\
            defeaters &    & defeater $|$ defeater defeaters\\
            defeater &   & \sleeckeyword{unless} boolExpr [\sleeckeyword{then} response] \\
            numOp &   & + $|$ - $|$ * \\
            relOp &    & $<$ $|$ $>$ $|$ $<>$ $|$ $<=$ $|$ $>=$ $|$ = \\
            boolOp &    & \sleeckeyword{and} $|$ \sleeckeyword{or} \\
        \bottomrule
        \end{tabular}
     }
    \caption{\dsle grammar. The extension from \dsl~\cite{Getir-Yaman-et-al-23} grammar is highlighted in green. \hl{(correct the highlight for the underlined numeric type)}}
    \label{tab:sleecplus-gram}
\end{table}

==> review.tex <==
%review commands
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{ulem}

\newcommand{\ra}{$\rightarrow$}
\newcommand{\ugh}[1]{\textcolor{red}{\uwave{#1}}} % please rephrase
\newcommand{\ins}[1]{\textcolor{blue}{\uline{#1}}} % please insert
\newcommand{\del}[1]{\textcolor{red}{\sout{#1}}} % please delete
\newcommand{\chg}[2]{\textcolor{red}{\sout{#1}}{\ra}\textcolor{blue}{\uline{#2}}} % please change

% Put edit comments in a really ugly standout display
\usepackage{ifthen}
\newboolean{showcomments}
\setboolean{showcomments}{true} % toggle to show or hide \chapter{?}
\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fcolorbox{gray}{yellow}{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
  }
  \newcommand{\version}{\emph{\scriptsize$-$working$-$}}
  }
  {\newcommand{\nb}[2]{}
  \newcommand{\version}{}
  }

\newcommand{\lina}[1]{\nb{Lina}{\footnotesize #1}}
\newcommand{\marsha}[1]{\nb{Marsha}{\footnotesize #1}}
\newcommand{\sinem}[1]{\nb{Sinem}{\footnotesize #1}}
\newcommand{\gena}[1]{\nb{Gena\'ina}{\footnotesize #1}}
\newcommand{\radu}[1]{\nb{Gena\'ina}{\footnotesize #1}}
\newcommand{\todo}[1]{\nb{TODO}{\footnotesize #1}}
